Quantitative Evaluation of SPH in TIG Spot Welding

While the application of the Smoothed Particle Hydrodynamics (SPH) method for the modeling of welding processes has become increasingly popular in recent years, little is yet known about the quantitative predictive capability of this method. We propose a novel SPH model for the simulation of the tungsten inert gas (TIG) spot welding process and conduct a thorough comparison between our SPH implementation and two Finite Element Method (FEM) based models. In order to be able to quantitatively compare the results of our SPH simulation method with grid based methods we additionally propose an improved particle to grid interpolation method based on linear least-squares with an optional hole-filling pass which accounts for missing particles. We show that SPH is able to yield excellent results, especially given the observed deviations between the investigated FEM methods and as such, we validate the accuracy of the method for an industrially relevant engineering application.

==> ms-1.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0}%
}%


==> sources/ansys.tex <==

For the benchmark, originally a comparison with Ansys CFX was planned. However, the transient simulation failed after time step 0.3[s], as pressure instabilities developed, see Figure \ref{fig:Ansys_C5*10^10_pres_0.3s}. The pressure instabilites originated from the momentum sink approach, which was modelled as porous loss, according to the recommendations in the Ansys Modelling Guide. The calculation would successfully finish when the value of the morphological constant was reduced to $C=5 \cdot 10^{7} \frac{kg}{m^{3} s}$. However, in this case the fluid motion in the solidified region was not negligible, see Figure \ref{fig:Ansys_C5*10^7_velo_1s} and a considerable discrepancy between Ansys CFX and the FEM aproach, as well as Ansys CFX and the SPH approach was detected, see for example the depth in Figure \ref{fig:Ansys_C5*10^7_temp_1s}. The mesh was composed of a 30°-wedge of a disc with symmetry boundary conditions along the axis-symmetry. It contained  182216 hexahedral elements, and the calculation time for the successful case with $C=5 \cdot 10^{7} \frac{kg}{m^{3} s}$ was around 30h for $2s$ of transient simulation on 12 cores of the RWTH-HPC-Cluster. However, it should be mentioned, that this solution time included the solution for electromagnetics.


\begin{figure}[ht]
    \centering
    \includegraphics[width=.4\textwidth]{img/ansys/highC_3000_full_pres.png}
    \caption{Simulation results from Ansys CFX, displaying pressure field in the cross section, at 0.3s, with $C=5 \cdot 10^{10}$. The simulation has become unstable.}
    \label{fig:Ansys_C5*10^10_pres_0.3s}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=.4\textwidth]{img/ansys/Sim08_sim_004_velo_1s.png}
    \caption{Simulation results from Ansys CFX, displaying velocity field in the cross section, at 1s, with $C=5 \cdot 10^{7}$. It can be seen that the velocities outside of the weld pool have not completely vanished}
    \label{fig:Ansys_C5*10^7_velo_1s}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.4\textwidth]{img/ansys/Sim08_sim_004_temp_1s.png}
    \caption{Simulation results from Ansys CFX, displaying temperature field in the cross section, at 1s, with $C=5 \cdot 10^{7}$. It can be seen that the depth of the weld pool is significantly larger than in the other two approaches at 1s }
    \label{fig:Ansys_C5*10^7_temp_1s}
\end{figure}


==> sources/relatedwork.tex <==
Das and Cleary \cite{DC16} use SPH in three-dimensional arc welding simulations in order to study temperature distributions flow patterns and plastic strain in the filler material and residual thermal stresses in the workpiece.
\sj{WCSPH, Tensile instability correction, Use Cauchy equation as basis, explicit euler cfl for both heat conduction and movement, }

Ito et al.~\cite{INI15} perform full simulations of TIG welding using the SPH method under consideration of flow driving forces. 
They show results for different material properties due to different sulphur contents and evaluate the flow patterns and the shape of the weld pool.
\sj{Domain Unbounded, no comparison to experiment or mesh, free surface}

Trautmann et al.~\cite{THF17} similarly perform weld pool simulations using SPH for a TIG welding process.
They consider gravity, bouyancy, viscosity and surface tension as flow driving forces and the arc pressure, shear and thermal effect were parametrized using experimental studies.
The penetration profiles of three different welding currents were compared to experimental results and show decent agreement.  
\sj{Unbounded domain, penetration profiles compared, free surface, temperature-dependent parameters (pretty much all of them), PCISPH}

A hybrid approach is investigated by Komen et al.~\cite{KTT20}, who use a Eulerian grid and Lagrangian particles in conjunction in order to simulate GMA welding. 
Molten metal is simulated by means of SPH, while the arc plasma and gas are simulated on a grid.
The methods are then weakly coupled and executed iteratively.

Komen et al.~\cite{KST18} also simulate the GMAW process under consideration of droplet formation and compare the weld pool shapes against experimental results.
In order to more easily visualize results they use an ensemble averaging in order to transfer particle data onto a regular grid.
